Subgroup Packing for Batched PASTA Transciphering

With transciphering, a server converts symmetrically encrypted records into homomorphic ciphertexts without learning the records or the symmetric key. For the PASTA cipher, this conversion involves dense linear maps whose implementation depends on how record words are arranged in the ciphertext. We ask whether rearranging a fixed batch can reduce its conversion cost. Instead of storing each record's words in a contiguous block, our layout interleaves records so that cyclic word shifts preserve each record's positions, which form a coset of a cyclic subgroup. For direct evaluation as a sum of masked translations, we characterize the required displacements and relate their counts, 255 for the contiguous layout and 128 for the subgroup layout, to a prior transversal-difference invariant. We implement three equally batched schedules for complete PASTA-3 conversion and subsequent public subset-sum queries in HElib. Across twelve paired corpora under six homomorphic keys, all 24 direct and subgroup conversions and all 48 subsequent queries return the expected values and required zeroes. The median paired ratio of direct to subgroup server cost is 1.60, including fresh public generation, conversion and two queries. The reduction comes with less remaining noise capacity. These results establish a packing-dependent cost--noise tradeoff.

==> source/macros.tex <==
\makeatletter
\newcommand{\tablerows}[1]{\@@input #1 }
\makeatother

\newcommand{\F}{\mathbb{F}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Qset}{Q}
\newcommand{\supp}{\operatorname{supp}}
\newcommand{\Gal}{\operatorname{Gal}}
\newcommand{\Dsize}{\operatorname{d}}
\newcommand{\betaBSGS}{\beta}
\newcommand{\code}[1]{\texttt{#1}}
\newcommand{\pastarepositoryreference}{Source repository; address withheld for anonymous review}
\newcolumntype{Y}{>{\raggedright\arraybackslash}X}
\newcolumntype{L}[1]{>{\raggedright\arraybackslash}p{#1}}

\makeatletter
\@ifundefined{c@theorem}{%
  \newtheorem{theorem}{Theorem}[section]
  \newtheorem{proposition}[theorem]{Proposition}
  \newtheorem{corollary}[theorem]{Corollary}
  \newtheorem{lemma}[theorem]{Lemma}
  \theoremstyle{definition}
  \newtheorem{definition}[theorem]{Definition}
  \newtheorem{example}[theorem]{Example}
  \newtheorem{remark}[theorem]{Remark}
}{}
\makeatother


==> tables/table1-affine-count-rows.tex <==
Contiguous direct, signed $15\times17$ & 30 & 255 & 0 \\
Contiguous composed, cyclic width 10 & 42 & 128 & 21 \\
Subgroup aligned, cyclic width 10 & 21 & 128 & 0 \\


==> tables/table2-conversion-rows.tex <==
Public generation & 0.093 [0.092, 0.112] & 0.093 [0.092, 0.112] \\
Conversion preparation & 28.333 [28.308, 28.434] & 17.309 [17.289, 17.338] \\
Conversion arithmetic & 7.502 [7.487, 7.520] & 4.774 [4.766, 4.787] \\
Complete conversion & 35.844 [35.790, 35.982] & 22.095 [22.076, 22.108] \\
Two complete queries & 0.684 [0.594, 0.802] & 0.708 [0.603, 0.822] \\
Recurring server total & 36.668 [36.565, 36.842] & 22.905 [22.812, 22.980] \\


==> tables/table3-capacity-outcome-rows.tex <==
460, paired & Contiguous direct & 78--81, Passed & 33--39, Passed \\
460, paired & Subgroup aligned & 76--78, Passed & 22--32, Passed \\
460, prior & Contiguous composed & -94, Refused & Not evaluated \\
400, prior & Contiguous direct & 23, Passed & -22, Refused \\
400, prior & Contiguous composed & -162, Refused & Not evaluated \\
400, prior & Subgroup aligned & 21, Passed & -32, Refused \\


==> tables/table4-query-rows.tex <==
Preparation & 196.84 [89.57, 244.16] & 202.61 [104.21, 274.50] \\
Encrypted arithmetic & 173.01 [171.36, 174.11] & 165.48 [164.24, 166.61] \\
Complete server query & 369.79 [260.22, 416.90] & 366.89 [273.93, 441.34] \\
Answer serialization & 2.73 [2.66, 2.94] & 2.56 [2.32, 2.62] \\
Decryption and all-slot decoding & 7167.98 [7114.56, 7198.71] & 7170.34 [7096.43, 7233.41] \\

